NARU: A Benchmark for NARrative Evolution and Cultural Nuance Understanding in Japanese Extreme Long Video

Long-form video understanding encompasses tasks that go beyond retrieving isolated events, including tracking an evolving narrative and interpreting social meaning that may remain implicit. However, existing benchmarks rarely evaluate these capabilities jointly, particularly in high-context, non-English media. To address this gap, we introduce NARU, a benchmark designed to evaluate Narrative evolution and Reasoning on cultural Understanding in Japanese long-form video. NARU consists of 1,481 questions grounded in 155 videos totaling 146.8 hours, spanning four narrative and five cultural dimensions. To construct the benchmark at this scale, we propose a hierarchical memory-based annotation pipeline that transforms raw video into structured event, narrative, and cultural annotations, then generates questions via task-oriented synthesis and iterative shortcut removal. The construction process includes two native-speaker verification stages involving 68 annotators. Evaluations across eight model configurations reveal substantial limitations in both long-range narrative integration and culturally grounded reasoning. By exposing these persistent gaps, NARU offers a systematic testing ground for developing MLLMs capable of reliably interpreting long-form, high-context video.

==> table/dataset_comparison.tex <==
\begin{table*}[t]
  \centering
  \caption{Comparison of {\ourbench} with representative video-understanding benchmarks. Average durations are reported in seconds when available. The primary focus summarizes the main evaluation target of each benchmark, including whether narrative evolution or culturally grounded interpretation is explicitly operationalized.}
  \label{tab:benchmark_comparison}
  \small
  \setlength{\tabcolsep}{4pt}
  \renewcommand{\arraystretch}{1.3}
  \begin{tabularx}{\textwidth}{@{}lrrr
    >{\centering\arraybackslash\hsize=0.75\hsize}X
    >{\centering\arraybackslash\hsize=1.25\hsize}X@{}}
    \toprule
    \textbf{Benchmark} & \textbf{\#Videos} & \textbf{Avg. sec.} & \textbf{\#QA} &
    \textbf{Annotation} & \textbf{Primary focus} \\
    \midrule
    MVBench~\cite{li2024mvbench} & 4,000 & 16 & 4,000 &
    Auto &
    Short-video temporal perception and action \\
    ActivityNet-QA~\cite{yu2019activitynet} & 5,800 & 180 & 58,000 &
    Human &
    Open-ended QA over complex web activities focusing on activity/event understanding. \\
    EgoSchema~\cite{mangalam2023egoschema} & 5,031 & 180 & 5,031 &
    Human &
    Egocentric long-horizon activity reasoning. \\
    MovieChat-1K~\cite{song2024moviechat} & 1,000 & 564 & 13,000 &
    Human &
    Movie-based long-video QA. Its narrative content is present but not organized as an explicit narrative-evolution taxonomy. \\
    MLVU~\cite{zhou2025mlvu} & 1,730 & 930 & 3,102 &
    Auto \& Human &
    Broad multi-task long-video understanding, including plot QA, ordering, and summarization. \\
    Video-MME~\cite{fu2025video} & 900 & 1,024 & 2,700 &
    Human &
    General video QA spanning perception, temporal understanding, and reasoning. \\
    LongVideoBench~\cite{wu2024longvideobench} & 3,763 & 473 & 6,678 &
    Human &
    Long-context referring reasoning over interleaved video. \\
    LVBench~\cite{wang2025lvbench} & 103 & 4,101 & 1,549 &
    Human &
    Long-video comprehension and information extraction. \\
    \midrule
    \textbf{\ourbench} & \textbf{155} & \textbf{3,408} & \textbf{1,483} &
    Auto \& native-speaker verified &
    Japanese long-form video understanding with explicit evaluation of both \textbf{narrative evolution} and \textbf{high-context cultural understanding}. \\
    \bottomrule
  \end{tabularx}
\end{table*}

% 16 ~\cite{jang2025videowebarena}\js{why a ref here?}



